Flavor Mixing Phenomenology in Supersymmetric Models

This dissertation investigates the flavor mixing effects in supersymmetric models on electroweak precision observables, Higgs boson mass predictions, B-physics observables, quark flavor violating Higgs decays, lepton flavor violating charged lepton decays and lepton flavor violating Higgs decays. The flavor mixing effects are studied in model independent way i.e. by putting off-diagonal entries in the sfermion mass matrix by hand as well as in the minimal flavor violating constrained MSSM, where mixing can originate from CKM matrix in the case of squarks and from PMNS matrix in the case of sleptons. We found that flavor mixing can have large impact to some observables, enabling us to put new constraints on parameter space in supersymmetric models.

==> paperdef.tex <==
\catcode`@=11
\def\citer{\@ifnextchar [{\@tempswatrue\@citexr}{\@tempswafalse\@citexr[]}}
 
\def\@citexr[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{--\penalty\@m}\@ifundefined
       {b@\@citeb}{{\bf ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
\hbox{\csname b@\@citeb\endcsname}}}{#1}}
\catcode`@=12

%\renewcommand{\topfraction}{1.0}
%\renewcommand{\bottomfraction}{0.3}
\renewcommand{\textfraction}{0}
\renewcommand{\floatpagefraction}{1.0}

% new commands for cross referencing
%\def\refeq#1{\mbox{(\ref{#1})}}
\def\refeq#1{\mbox{Eq.~(\ref{#1})}}
\def\refeqs#1{\mbox{Eqs.~(\ref{#1})}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\refta#1{\mbox{Tab.~\ref{#1}}}
%\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tabs.~\ref{#1}}}
%\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Sect.~\ref{#1}}}
\def\refses#1{\mbox{Sects.~\ref{#1}}}
%\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
%\def\refapp#1{\mbox{Appendix~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

\newcommand\eq{\; = \;}

\newcommand{\mEW}{m_{\rm SUSY-EW}}
\newcommand{\mQCD}{m_{\rm SUSY-QCD}}
\newcommand{\mD}{m_D}
\newcommand{\mM}{m_M}
\newcommand{\mL}{m_{\tilde L}}
\newcommand{\mR}{m_{\tilde R}}
\newcommand{\mst}{m_{\tilde{t}}}
\newcommand{\mstr}{m_{\tilde{t}_R}}
\newcommand{\mstl}{m_{\tilde{t}_L}}
\newcommand{\mste}{m_{\tilde{t}_1}}
\newcommand{\mstz}{m_{\tilde{t}_2}}
\newcommand{\msti}{m_{\tilde{t}_i}}
\newcommand{\mstj}{m_{\tilde{t}_j}}
\newcommand{\msb}{m_{\tilde{b}}}
\newcommand{\msbr}{m_{\tilde{b}_R}}
\newcommand{\msbl}{m_{\tilde{b}_L}}
\newcommand{\msbe}{m_{\tilde{b}_1}}
\newcommand{\msbeOS}{m_{\tilde{b}_{1,{\rm OS}}}}
\newcommand{\msbz}{m_{\tilde{b}_2}}
\newcommand{\msbi}{m_{\tilde{b}_i}}
\newcommand{\msbj}{m_{\tilde{b}_j}}
\newcommand{\mstau}{m_{\tilde{\tau}}}
\newcommand{\MstL}{M_{\tilde{t}_L}}
\newcommand{\MstR}{M_{\tilde{t}_R}}
\newcommand{\MsbL}{M_{\tilde{b}_L}}
\newcommand{\MsbR}{M_{\tilde{b}_R}}
\newcommand{\MsqL}{M_{\tilde{q}_L}}
\newcommand{\MsqR}{M_{\tilde{q}_R}}
\newcommand{\At}{A_t}
\newcommand{\Ab}{A_b}
\newcommand{\Ac}{A_c}
\newcommand{\As}{A_s}
\newcommand{\Au}{A_u}
\newcommand{\Ad}{A_d}
\newcommand{\Atau}{A_\tau}
\newcommand{\Anu}{A_\nu}
\newcommand{\Aq}{A_q}
\newcommand{\Xt}{X_t}
\newcommand{\Xb}{X_b}
\newcommand{\Xq}{X_q}
\newcommand{\Xc}{X_c}
\newcommand{\Xs}{X_s}
\newcommand{\Xu}{X_u}
\newcommand{\Xd}{X_d}
\newcommand{\Bnu}{B_\nu}
\newcommand{\mnu}{m_\nu}
\newcommand{\Ynu}{Y_\nu}
\def\tif{\tilde f}
\def\tiu{\tilde u}
\def\tid{\tilde d}
\def\tiq{\tilde q}
\def\til{\tilde l}
\def\tinu{\tilde \nu}
 \newcommand{\mf}{m_f}
\newcommand{\msfr}{m_{\tilde{f}_R}}
\newcommand{\msfl}{m_{\tilde{f}_L}}
\newcommand{\msf}{m_{\tilde{f}}}
\newcommand{\msfi}{m_{\tilde{f}_i}}
\newcommand{\msfe}{m_{\tilde{f}_1}}
\newcommand{\msfz}{m_{\tilde{f}_2}}

%\newcommand{\ms}{M_S}
%\newcommand{\msusy}{M_{\rm SUSY}}
\newcommand{\msusy}{m_{\rm SUSY}}
\newcommand{\msq}{m_{\tilde{q}}}
\newcommand{\msqi}{m_{\tilde{q}_i}}
\newcommand{\msqip}{m_{\tilde{q}_{i'}}}
\newcommand{\msqj}{m_{\tilde{q}_j}}
\newcommand{\msqe}{m_{\tilde{q}_1}}
\newcommand{\msqz}{m_{\tilde{q}_2}}

\newcommand{\Sf}{\tilde{f}}
\newcommand{\sfl}{\tilde{f}_L}
\newcommand{\sfr}{\tilde{f}_R}
\newcommand{\sfe}{\tilde{f}_1}
\newcommand{\sfz}{\tilde{f}_2}
\newcommand{\sfi}{\tilde{f}_i}
\newcommand{\sfj}{\tilde{f}_j}
\newcommand{\sfez}{\tilde{f}_{12}}
\newcommand{\sfze}{\tilde{f}_{21}}

%\newcommand{\Hi}{H_i}
\newcommand{\Hi}{h_i}
\newcommand{\cHe}{\cH_1}
\newcommand{\cHz}{\cH_2}
%\newcommand{\He}{H_1}
\newcommand{\He}{h_1}
%\newcommand{\Hz}{H_2}
\newcommand{\Hz}{h_2}
%\newcommand{\Hd}{H_3}
\newcommand{\Hd}{h_3}
\newcommand{\mHe}{m_{\He}}
\newcommand{\mHz}{m_{\Hz}}
\newcommand{\mHd}{m_{\Hd}}
\newcommand{\MHe}{M_{\He}}
\newcommand{\MHz}{M_{\Hz}}
\newcommand{\MHd}{M_{\Hd}}
\newcommand{\Pe}{\phi_1}
\newcommand{\Pz}{\phi_2}
\newcommand{\Pez}{\phi_{1,2}}
\newcommand{\PePz}{\phi_1\phi_2}
\newcommand{\mpe}{m_{\Pe}}
\newcommand{\mpz}{m_{\Pz}}
\newcommand{\mpez}{m_{\PePz}}
% \newcommand{\smallz}{{\scriptscriptstyle Z}} %  a smaller Z
% \newcommand{\smallD}{{\scriptscriptstyle D}} %
% \newcommand{\smallQ}{{\scriptscriptstyle Q}} %
% \newcommand{\smallU}{{\scriptscriptstyle U}} %

\def\unity{{\rm 1\mskip-4.25mu l}}
\newcommand{\CMSSMI}{CMSSM-seesaw~I}
\newcommand{\SU}{\mathrm {SUSY}}
\newcommand{\SM}{\mathrm {SM}}
\newcommand{\os}{\mathrm {OS}}
\newcommand{\hi}{\mathrm {Higgs}}
\def\Liz#1{{\rm Li}_2 \KL #1 \KR}
\newcommand{\msbar}{$\overline{\rm{MS}}$}
\newcommand{\msbarm}{\overline{\rm{MS}}}
\newcommand{\drbar}{$\overline{\rm{DR}}$}
\newcommand{\drbarm}{\overline{\rm{DR}}}
\newcommand{\DRbar}{\ensuremath{\overline{\mathrm{DR}}}}
\newcommand{\mDRbar}{\ensuremath{\mathrm{m}\overline{\mathrm{DR}}}}
\newcommand{\MSbar}{\ensuremath{\overline{\mathrm{MS}}}}
\newcommand{\MSbarb}{\ensuremath{\overline{\mathbf{MS}}}}
\newcommand{\OS}{\mathrm{OS}}
\newcommand{\mudim}{\mu_{\DRbar}}
\def\order#1{\ensuremath{{\cal O}(#1)}}
\newcommand{\cp}{{\cal CP}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cHi}{{\cal H}_i}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cZ}{{\cal Z}}
\newcommand{\wz}{\sqrt{2}}
\newcommand{\edz}{\frac{1}{2}}
\def\ed#1{\frac{1}{#1}}
\newcommand{\twol}{two-loop}
\newcommand{\onel}{one-loop}
\newcommand{\mma}{{\em Mathematica}}
\newcommand{\tc}{{\tt TwoCalc}}
\newcommand{\fa}{{\tt FeynArts}}
\newcommand{\fc}{{\tt FormCalc}}
\newcommand{\fh}{{\tt FeynHiggs}}
\newcommand{\fhto}{{\em FeynHiggs2.1}}
\newcommand{\fhtt}{{\tt FeynHiggs\,2.5}}
\newcommand{\fhf}{{\em FeynHiggsFast}}
\newcommand{\fhfc}{{\em FeynHiggsFastC}}
\newcommand{\cpsh}{{\em CPsuperH}}
\newcommand{\rp}{$\rho\,$-parameter}

\newcommand{\MW}{M_W}
\newcommand{\MZ}{M_Z}
\newcommand{\mA}{m_A}
\newcommand{\MA}{M_A}
\newcommand{\mh}{m_h}
\newcommand{\mhtree}{m_{h,{\rm tree}}}
\newcommand{\mH}{m_H}
\newcommand{\mHtree}{m_{H,{\rm tree}}}
\newcommand{\Mh}{M_h}
\newcommand{\MH}{M_H}
\newcommand{\MHp}{M_{H^\pm}}
\newcommand{\MHpm}{M_{H^\pm}}
\newcommand{\mHp}{m_{H^\pm}}
%\newcommand{\mHp}{M_{H^\pm}}
\newcommand{\MHpq}{\bar{M}_{H^\pm}}
\newcommand{\mhH}{m_{hH}}
\newcommand{\mHh}{m_{Hh}}
\newcommand{\mhA}{m_{hA}}
\newcommand{\mhG}{m_{hG}}
%\newcommand{\mH}{m_H}
\newcommand{\mHA}{m_{HA}}
\newcommand{\mHG}{m_{HG}}
\newcommand{\mAG}{m_{AG}}
\newcommand{\mG}{m_G}
\newcommand{\mHpm}{m_{H^\pm}}
\newcommand{\mHmGp}{m_{H^- G^+}}
\newcommand{\mGmHp}{m_{G^- H^+}}
\newcommand{\mGp}{m_{G^\pm}}
\newcommand{\mGpm}{m_{G^\pm}}
\newcommand{\mHtr}{m_{H(0)}}
\newcommand{\mhtr}{m_{h(0)}}
\newcommand{\mGtr}{m_{G(0)}}
\newcommand{\mAtr}{m_{A(0)}}
\newcommand{\mHpmtr}{m_{H^\pm(0)}}
\newcommand{\mGpmtr}{m_{G^\pm(0)}}
\newcommand{\mhmax}{$\mh^{\rm max}$}

\newcommand{\mt}{m_t}
\newcommand{\mtms}{\overline{m}_t}
\newcommand{\mq}{m_{q}}
\newcommand{\mb}{m_{b}}
\newcommand{\mbbar}{\overline{m}_b}
\newcommand{\mc}{m_c}
\newcommand{\ms}{m_s}
\newcommand{\mup}{m_u}
\newcommand{\md}{m_d}
\newcommand{\mtau}{m_{\tau}}
\newcommand{\gl}{\tilde{g}}
\newcommand{\Mgl}{m_{\tilde{g}}}
\newcommand{\mgl}{m_{\tilde{g}}}
\newcommand{\Sferm}{\tilde{f}}
\newcommand{\Sfermp}{\tilde{f}'}
\newcommand{\sq}{\tilde{q}}
\newcommand{\sqi}{\tilde{q}_i}
\newcommand{\sqj}{\tilde{q}_j}
\newcommand{\sql}{\tilde{q}_L}
\newcommand{\sqr}{\tilde{q}_R}
\newcommand{\sqe}{\tilde{q}_1}
\newcommand{\sqz}{\tilde{q}_2}
\newcommand{\Stop}{\tilde{t}}
\newcommand{\StopL}{\tilde{t}_L}
\newcommand{\StopR}{\tilde{t}_R}
\newcommand{\Stope}{\tilde{t}_1}
\newcommand{\Stopz}{\tilde{t}_2}
\newcommand{\Stopi}{\tilde{t}_i}
\newcommand{\Stopj}{\tilde{t}_j}
\newcommand{\Sbot}{\tilde{b}}
\newcommand{\SbotL}{\tilde{b}_L}
\newcommand{\SbotR}{\tilde{b}_R}
\newcommand{\Sbote}{\tilde{b}_1}
\newcommand{\Sbotz}{\tilde{b}_2}
\newcommand{\Sboti}{\tilde{b}_i}
\newcommand{\Sbotj}{\tilde{b}_j}
\newcommand{\Scha}{\tilde{c}}
\newcommand{\SchaL}{\tilde{c}_L}
\newcommand{\SchaR}{\tilde{c}_R}
\newcommand{\Sstr}{\tilde{s}}
\newcommand{\SstrL}{\tilde{s}_L}
\newcommand{\SstrR}{\tilde{s}_R}
\newcommand{\Sup}{\tilde{u}}
\newcommand{\SupL}{\tilde{u}_L}
\newcommand{\SupR}{\tilde{u}_R}
\newcommand{\Sdown}{\tilde{d}}
\newcommand{\SdownL}{\tilde{d}_L}
\newcommand{\SdownR}{\tilde{d}_R}
\newcommand{\Stau}{\tilde{\tau}}
\newcommand{\Staue}{\tilde{\tau}_1}
\newcommand{\AStaue}{\bar{\tilde{\tau}}_1}
\newcommand{\Snet}{\tilde{\nu}_\tau}
\newcommand{\Smu}{\tilde \mu}
%new MJ
\newcommand{\SuL}{\tilde {u}_L}
\newcommand{\ScL}{\tilde {c}_L}
\newcommand{\StL}{\tilde {t}_L}
\newcommand{\SdL}{\tilde {d}_L}
\newcommand{\SsL}{\tilde {s}_L}
\newcommand{\SbL}{\tilde {b}_L}
\newcommand{\SuR}{\tilde {u}_R}
\newcommand{\ScR}{\tilde {c}_R}
\newcommand{\StR}{\tilde {t}_R}
\newcommand{\SdR}{\tilde {d}_R}
\newcommand{\SsR}{\tilde {s}_R}
\newcommand{\SbR}{\tilde {b}_R}
\newcommand{\SfL}{\tilde {f}_L}
\newcommand{\SfR}{\tilde {f}_R}

\newcommand{\Sel}{\tilde e}
\newcommand{\SelL}{\tilde {e}_L}
\newcommand{\SelR}{\tilde {e}_R}
\newcommand{\StauL}{\tilde{\tau}_L}
\newcommand{\StauR}{\tilde{\tau}_R}
\newcommand{\SmuL}{\tilde{\mu}_L}
\newcommand{\SmuR}{\tilde{\mu}_R}
\newcommand{\Snu}{\tilde \nu}
\newcommand{\SNu}{\tilde N}
\newcommand{\Sneum}{\tilde \nu_\mu}
\newcommand{\db}{\De_b}
\newcommand{\dst}{\Delta_{\tilde{t}}}
\newcommand{\tst}{\theta_{\tilde{t}}}
\newcommand{\tsb}{\theta_{\tilde{b}}}
\newcommand{\tsf}{\theta\kern-.20em_{\tilde{f}}}
\newcommand{\tsfp}{\theta\kern-.20em_{\tilde{f}\prime}}
\newcommand{\tsq}{\theta\kern-.15em_{\tilde{q}}}
%\newcommand{\sw}{s_W}
%\newcommand{\cw}{c_W}
\newcommand{\sweff}{\sin^2\theta_{\mathrm{eff}}}

\newcommand{\cha}[1]{\tilde \chi^\pm_{#1}}
\newcommand{\chap}[1]{\tilde \chi^+_{#1}}
\newcommand{\cham}[1]{\tilde \chi^-_{#1}}
\newcommand{\mcha}[1]{m_{\tilde \chi^\pm_{#1}}}
\newcommand{\neu}[1]{\tilde \chi^0_{#1}}
\newcommand{\mneu}[1]{m_{\tilde \chi^0_{#1}}}

\newcommand{\sintt}{\sin\tst}
\newcommand{\sinQtt}{\sin^2\tst}
\newcommand{\sinZtt}{\sin 2\tst}
\newcommand{\sinQZtt}{\sin^2 2\tst}
\newcommand{\sintb}{\sin\tsb}
\newcommand{\sinQtb}{\sin^2\tsb}
\newcommand{\sinZtb}{\sin 2\tsb}
\newcommand{\sintf}{\sin\tsf}
\newcommand{\sintfp}{\sin\tsfp}
\newcommand{\sinQtf}{\sin^2\tsf}
\newcommand{\sinZtf}{\sin 2\tsf}
\newcommand{\sintq}{\sin\tsq}
\newcommand{\sinQtq}{\sin^2\tsq}
\newcommand{\sinZtq}{\sin 2\tsq}

\newcommand{\costt}{\cos\tst}
\newcommand{\cosQtt}{\cos^2\tst}
\newcommand{\cosZtt}{\cos 2\tst}
\newcommand{\costb}{\cos\tsb}
\newcommand{\cosQtb}{\cos^2\tsb}
\newcommand{\cosZtb}{\cos 2\tsb}
\newcommand{\costf}{\cos\tsf}
\newcommand{\costfp}{\cos\tsfp}
\newcommand{\cosQtf}{\cos^2\tsf}
\newcommand{\cosZtf}{\cos 2\tsf}
\newcommand{\costq}{\cos\tsq}
\newcommand{\cosQtq}{\cos^2\tsq}
\newcommand{\cosZtq}{\cos 2\tsq}

\newcommand{\stt}{s_{\tilde{t}}}
\newcommand{\stb}{s_{\tilde{b}}}
\newcommand{\stf}{s_{\tilde{f}}}
\newcommand{\stq}{s_{\tilde{q}}}
\newcommand{\ctt}{c_{\tilde{t}}}
\newcommand{\ctb}{c_{\tilde{b}}}
\newcommand{\ctf}{c_{\tilde{f}}}
\newcommand{\ctq}{c_{\tilde{q}}}

\newcommand{\KL}{\left(}
\newcommand{\KR}{\right)}
\newcommand{\KKL}{\left[}
\newcommand{\KKR}{\right]}
\newcommand{\KKKL}{\left\{}
\newcommand{\KKKR}{\right\}}
\newcommand{\BL}{\lbrack}
\newcommand{\BR}{\rbrack}

\newcommand{\VL}{\left( \begin{array}{c}}
\newcommand{\VR}{\end{array} \right)}
\newcommand{\ML}{\left( \begin{array}{cc}}
\newcommand{\MLd}{\left( \begin{array}{ccc}}
\newcommand{\MLv}{\left( \begin{array}{cccc}}
\newcommand{\MR}{\end{array} \right)}
\newcommand{\hc}{\mbox {h.c.}}
\newcommand{\re}{\mathop{\mathrm{Re}}}
\newcommand{\im}{\mathop{\mathrm{Im}}}
\newcommand{\wt}{\widetilde}
\newcommand{\wtre}{\widetilde\re}
\newcommand{\wtim}{\widetilde\im}
\newcommand{\OP}{\omega_+}
\newcommand{\OM}{\omega_-}
\newcommand{\Tb}{\tan \beta}
\newcommand{\tb}{\tan \beta}
\newcommand{\TQb}{\tan^2 \beta}
\newcommand{\CTb}{\cot \beta}
\newcommand{\CTQb}{\cot^2 \beta}
%\newcommand{\Sb}{\sin \beta}
\newcommand{\Sbe}{\sin \beta}
\newcommand{\sbe}{s_\be}
\newcommand{\SQb}{\sin^2\beta}
\newcommand{\SDb}{\sin^3\beta}
\newcommand{\SVb}{\sin^4\beta}
\newcommand{\Cb}{\cos \beta}
\newcommand{\cbe}{c_\be}
\newcommand{\CQb}{\cos^2\beta}
\newcommand{\CDb}{\cos^3\beta}
\newcommand{\CVb}{\cos^4\beta}
\newcommand{\Sa}{\sin \alpha}
\newcommand{\sa}{s_\al}
\newcommand{\SQa}{\sin^2\alpha}
\newcommand{\Ca}{\cos \alpha}
\newcommand{\ca}{c_\al}
\newcommand{\CQa}{\cos^2\alpha}
\newcommand{\Ta}{\tan\al}
\newcommand{\CTa}{\cot\al}
\newcommand{\Sab}{\sin (\alpha + \beta)}
\newcommand{\Cab}{\cos (\alpha + \beta)}
\newcommand{\Sba}{\sin (\beta - \alpha)}
\newcommand{\Samb}{\sin (\al - \be)}
\newcommand{\Cba}{\cos (\beta - \alpha)}
\newcommand{\Camb}{\cos (\al - \be)}
\newcommand{\SZa}{\sin 2\alpha}
\newcommand{\SQZa}{\sin^2 2\alpha}
\newcommand{\CZa}{\cos 2\alpha}
\newcommand{\CQZa}{\cos^2 2\alpha}
\newcommand{\SZb}{\sin 2\beta}
\newcommand{\SQZb}{\sin^2 2\beta}
\newcommand{\CZb}{\cos 2\beta}
\newcommand{\CQZb}{\cos^2 2\beta}
\newcommand{\CDZb}{\cos^3 2\beta}
\newcommand{\CVZb}{\cos^4 2\beta}
\newcommand{\CQba}{\cos^2 (\beta - \alpha)}
\newcommand{\SQba}{\sin^2 (\beta - \alpha)}
\newcommand{\SDba}{\sin^3 (\beta - \alpha)}
\newcommand{\CQab}{\cos^2 (\alpha + \beta)}
\newcommand{\SQab}{\sin^2 (\alpha + \beta)}
\newcommand{\SDab}{\sin^3 (\alpha + \beta)}
\newcommand{\SDea}{\sin \De\al}
\newcommand{\CDea}{\cos \De\al}
\newcommand{\CQDea}{\cos^2\De\al}
\newcommand{\TDea}{\tan \De\al}
\newcommand{\TQDea}{\tan^2\De\al}

\newcommand{\tev}{\,\, \mathrm{TeV}}
\newcommand{\gev}{\,\, \mathrm{GeV}}
\newcommand{\mev}{\,\, \mathrm{MeV}}
\newcommand{\ev}{\,\, \mathrm{eV}}

\newcommand{\BC}{\begin{center}}
\newcommand{\EC}{\end{center}}
\newcommand{\BE}{\begin{equation}}
\newcommand{\EE}{\end{equation}}
\newcommand{\BEA}{\begin{eqnarray}}
%\newcommand{\BEAnn}{\begin{eqnarray*}}
\newcommand{\EEA}{\end{eqnarray}}
%\newcommand{\EEAnn}{\end{eqnarray*}}
\newcommand{\non}{\nonumber}
\newcommand{\id}{{\rm 1\kern-.12em
\rule{0.3pt}{1.5ex}\raisebox{0.0ex}{\rule{0.1em}{0.3pt}}}}
\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}

\newcommand{\matr}[1]{{\mathbf{#1}}}
\newcommand{\musteq}{\stackrel{!}{=}}
\newcommand{\setR}{\ensuremath{\mathbb{R}}}
\newcommand{\setC}{\ensuremath{\mathbb{C}}}
\newcommand{\VHiggs}{V_H}
\newcommand{\FirstOrder}{\mathcal{O}_{(1)}}
\newcommand{\SecondOrder}{\mathcal{O}_{(2)}}
\newcommand{\tstop}{$t$-$\tilde{t}$}
\newcommand{\bsbot}{$b$-$\tilde{b}$}
\newcommand{\fsf}{$f$-$\tilde{f}$}
\newcommand{\pzero}{$p^2$=0}
\newcommand{\MSusy}{M_{\mathrm{Susy}}}
\newcommand{\MOne}{M_1}
\newcommand{\MTwo}{M_2}
\newcommand{\MThree}{M_3}
\newcommand{\mGl}{m_{\tilde{g}}}
\newcommand{\absXt}{|X_t|}
\newcommand{\argXt}{\arg(X_t)}
\newcommand{\reXt}{\Re X_t}
\newcommand{\imXt}{\Im X_t}

\newcommand{\reAt}{\Re A_t}
\newcommand{\imAt}{\Im A_t}
\newcommand{\absAt}{|A_t|}
\newcommand{\argAt}{\arg(A_t)}

\newcommand{\reA}{\Re A_0}
\newcommand{\imA}{\Im A_0}
\newcommand{\absA}{|A_0|}
\newcommand{\argA}{\arg(A_0)}

\newcommand{\absmu}{|\mu|}
\newcommand{\argmu}{\arg(\mu)}

\newcommand{\mphi}{m_\phi}
\newcommand{\Dmphi}{\De \mphi}
\newcommand{\Dmh}{\De \mh}
\newcommand{\DmH}{\De \mH}
\newcommand{\DmHp}{\De \mHp}
\newcommand{\mHol}{m_{H(1)}}
\newcommand{\mhol}{m_{h(1)}}
\newcommand{\mAol}{m_{A(1)}}
\newcommand{\dmhol}{\Delta m_{h(1)}}
\newcommand{\mHone}{m_{H_1}}
\newcommand{\mHtwo}{m_{H_2}}
\newcommand{\mHthree}{m_{H_3}}
\newcommand{\dmtt}{\Delta m_{32}}
\newcommand{\mHtl}{m_{H(2)}}
\newcommand{\mhtl}{m_{h(2)}}
\newcommand{\mHpmol}{m_{H^\pm(1)}}

\newcommand{\tadH}{T_H}
\newcommand{\tadh}{T_h}
\newcommand{\tadA}{T_A}
\newcommand{\tadG}{T_G}
\newcommand{\tanb}{\tan \beta\,}
\newcommand{\sinb}{\sin \beta\,}
\newcommand{\cosb}{\cos \beta\,}
\newcommand{\sinbsq}{\sin^2 \!\beta\,}
\newcommand{\cosbsq}{\cos^2 \!\beta\,}
\newcommand{\sina}{\sin \alpha\,}
\newcommand{\cosa}{\cos \alpha\,}
\newcommand{\tana}{\tan \alpha\,}
\newcommand{\sinasq}{\sin^2 \!\alpha\,}
\newcommand{\cosasq}{\cos^2 \!\alpha\,}
\newcommand{\sw}{s_\mathrm{w}}
\newcommand{\cw}{c_\mathrm{w}}
\newcommand{\betan}{\beta_\mathrm{n}}
\newcommand{\betac}{\beta_\mathrm{c}}

\newcommand{\dmZsq}{\delta m_Z^2}
\newcommand{\dMZsq}{\delta \MZ^2}
\newcommand{\dmWsq}{\delta m_W^2}
\newcommand{\dMWsq}{\delta \MW^2}
\newcommand{\dmhsq}{\delta m_h^2}
\newcommand{\dmhHsq}{\delta m_{hH}^2}
\newcommand{\dmHhsq}{\delta m_{Hh}^2}
\newcommand{\dmhGsq}{\delta m_{hG}^2}
\newcommand{\dmhAsq}{\delta m_{hA}^2}
\newcommand{\dmHsq}{\delta m_H^2}
\newcommand{\dmHGsq}{\delta m_{HG}^2}
\newcommand{\dmHAsq}{\delta m_{HA}^2}
\newcommand{\dmAsq}{\delta m_A^2}
\newcommand{\dmAGsq}{\delta m_{AG}^2}
\newcommand{\dmGsq}{\delta m_G^2}
\newcommand{\dmHpmsq}{\delta m_{H^\pm}^2}
\newcommand{\dmHmGpsq}{\delta m_{H^- G^+}^2}
\newcommand{\dmGmHpsq}{\delta m_{G^- H^+}^2}
\newcommand{\dmGpmsq}{\delta m_{G^\pm}^2}

\newcommand{\dtadH}{\delta T_H}
\newcommand{\dtadh}{\delta T_h}
\newcommand{\dtadA}{\delta T_A}

\newcommand{\dtanb}{\delta\!\tan\!\beta\,}
\newcommand{\dZ}[1]{\delta Z_{#1}}

\newcommand{\dd}{\partial\,}



\newcommand{\cf}{C_F}
\newcommand{\gf}{G_F}
\newcommand{\nf}{N_f}
% shorthands for greek letters
\def\al{\alpha}
\def\acp{\al_\cp}
\def\aeff{\al_{\rm eff}}
\def\aeffapprox{\al_{\rm eff}{\rm (approx)}}
\newcommand{\Saeff}{\sin\aeff}
\newcommand{\Caeff}{\cos\aeff}
\def\als{\alpha_s}
\def\alt{\alpha_t}
\def\alb{\alpha_b}
\def\altl{\alpha_{\rm 2-loop}}
\def\gs{g_s}
\def\be{\beta}
\def\ben{\be_0}
\def\bee{\be_1}
\def\bez{\be_2}
\def\ga{\gamma}
\def\gan{\ga_0}
\def\gae{\ga_1}
\def\gaz{\ga_2}
\def\de{\delta}
\newcommand{\deABij}{\de^{AB}_{ij}}
\newcommand{\deFABij}{\de^{FAB}_{ij}}
\newcommand{\del}[2]{\de^{#1}_{#2}}
\def\deqed{\de\Ga_\ga}
\def\eps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\ie{i\epsilon}
\def\om{\omega}
\def\Ga{\Gamma}
\def\Gh{\Ga_h}
\def\GH{\Ga_H}
\def\Gz{\Ga_0}
\def\Ge{\Ga_1}
%\def\Geeff{\Ga_{1,\rm eff}}
%\def\Geg{\Ga_{1,g}}
%\def\Gga{\Ga_\ga}
%\def\Gg{\Ga_g}
%\def\Ggl{\Ga_{\gl}}
\def\Gtot{\Ga_{\rm tot}}
\def\De{\Delta}
%\def\Deca{\De_{H^\pm A}}
\def\La{\Lambda}
\def\Laqcd{\La_{\rm QCD}}
\def\Si{\Sigma}
\def\Sip{\Sigma'}
\newcommand{\ddiv}{|_{\rm div}}
% \def\Sie{\Sigma^{(1)}}
% \def\Siz{\Sigma^{(2)}}
% \def\Sii{\Sigma^{(i)}}
% \def\Siep{\Sigma'^{(1)}}
% \def\Sizp{\Sigma'^{(2)}}
% \def\Siip{\Sigma'^{(i)}}
\def\phixt{\varphi_{\Xt}}
\def\phiat{\varphi_{\At}}
\def\phiab{\varphi_{\Ab}}
\def\phiatau{\varphi_{\Atau}}
\def\phia{\varphi_{A}}
\def\phimu{\varphi_{\mu}}
\def\phiMe{\varphi_{M_1}}
\def\phiMz{\varphi_{M_2}}
\def\phigl{\varphi_{\gl}}

\def\hSi{\hat{\Sigma}}
\newcommand{\se}[1]{\Sigma_{#1}}
\newcommand{\ser}[1]{\hat{\Sigma}_{#1}}
\def\hSip{\hat{\Sigma}'}
\def\Sip{\Sigma'}
% \def\hSie{\hat{\Sigma}^{(1)}}
% \def\hSiz{\hat{\Sigma}^{(2)}}
% \def\hSiep{\hat{\Sigma}^{(1)}'}
% \def\hSizp{\hat{\Sigma}^{(2)}'}
% \def\hSiH{\hSi_{HH}}
% \def\hSih{\hSi_{hh}}
% \def\hSihH{\hSi_{hH}}
% \def\SiH{\Si_{HH}}
% \def\Sih{\Si_{hh}}
% \def\SihH{\Si_{hH}}
% \def\hSipH{\hSip_{HH}}
% \def\hSiph{\hSip_{hh}}
% \def\hSiphH{\hSip_{hH}}
% \def\hSieh{\hSie_{h}}
% \def\hSieH{\hSie_{H}}
% \def\hSiehH{\hSie_{hH}}
% \def\hSizh{\hSiz_{h}}
% \def\hSizH{\hSiz_{H}}
% \def\hSizhH{\hSiz_{hH}}
\newcommand{\htad}{\hat{t}}
\newcommand{\tade}{t^{(1)}}
\newcommand{\tadz}{t^{(2)}}

% \newcommand{\Ph}{\mathswitchr h}
% \newcommand{\PH}{\mathswitchr H}

% \newcommand{\deMZe}{\de \MZ^{2\,(1)}}
% \newcommand{\deMZz}{\de \MZ^{2\,(2)}}
% \newcommand{\deMZi}{\de \MZ^{2\,(i)}}
% \newcommand{\deMAe}{\de \MA^{2\,(1)}}
% \newcommand{\deMAz}{\de \MA^{2\,(2)}}
% \newcommand{\deMAi}{\de \MA^{2\,(i)}}
% \newcommand{\deZHie}{\de Z_{H_i}^{(1)}}
% \newcommand{\deZHiz}{\de Z_{H_i}^{(2)}}
% \newcommand{\deZHee}{\de Z_{H_1}^{(1)}}
% \newcommand{\deZHez}{\de Z_{H_1}^{(2)}}
% \newcommand{\deZHze}{\de Z_{H_2}^{(1)}}
% \newcommand{\deZHzz}{\de Z_{H_2}^{(2)}}
% \newcommand{\deTbe}{\de\Tb^{(1)}}
% \newcommand{\deTbz}{\de\Tb^{(2)}}
% \newcommand{\detie}{\de t_i^{(1)}}
% \newcommand{\detiz}{\de t_i^{(2)}}
% \newcommand{\detee}{\de t_1^{(1)}}
% \newcommand{\detez}{\de t_1^{(2)}}
% \newcommand{\detei}{\de t_1^{(i)}}
% \newcommand{\detze}{\de t_2^{(1)}}
% \newcommand{\detzz}{\de t_2^{(2)}}
% \newcommand{\detzi}{\de t_2^{(i)}}
% \newcommand{\deVie}{\de V_i^{(1)}}
% \newcommand{\deViz}{\de V_i^{(2)}}
% \newcommand{\deVee}{\de V_{\Pe}^{(1)}}
% \newcommand{\deVez}{\de V_{\Pe}^{(2)}}
% \newcommand{\deVei}{\de V_{\Pe}^{(i)}}
% \newcommand{\deVze}{\de V_{\Pz}^{(1)}}
% \newcommand{\deVzz}{\de V_{\Pz}^{(2)}}
% \newcommand{\deVzi}{\de V_{\Pz}^{(i)}}
% \newcommand{\deVeze}{\de V_{\PePz}^{(1)}}
% \newcommand{\deVezz}{\de V_{\PePz}^{(2)}}
% \newcommand{\deVezi}{\de V_{\PePz}^{(i)}}


% \newcommand{\SLASH}[2]{\makebox[#2ex][l]{$#1$}/}
% \newcommand{\Dslash}{\SLASH{D}{.5}\,}
% \newcommand{\dslash}{\SLASH{\dd}{.15}}
% \newcommand{\kslash}{\SLASH{k}{.15}}
% \newcommand{\pslash}{\SLASH{p}{.2}}
% \newcommand{\qslash}{\SLASH{q}{.08}}

% \newcommand{\sqmsmt}{\sqrt{\ms^2-\mt^2}}
% \newcommand{\sqmsmtbar}{\sqrt{\ms^2-\mtms^2}}
% \newcommand{\lmtms}{\KL\frac{\mt^2}{\ms^2}\KR}
% \newcommand{\lmtmsms}{\KL\frac{\mtms^2}{\ms^2}\KR}
% \newcommand{\lmsmt}{\KL\frac{\ms^2 - \mt^2}{\mt^2}\KR}

% \newcommand{\lc}{linear collider}
% \newcommand{\epem}{$e^+e^-$}
% \newcommand{\eetohZhA}{$e^+e^- \to hZ,hA$}
% \newcommand{\eetohZ}{$e^+e^- \to hZ$}
% \newcommand{\eetohA}{$e^+e^- \to hA$}
% \newcommand{\ipb}{$\mbox{pb}^{-1}$}
% \newcommand{\ifb}{$\mbox{fb}^{-1}$}
% \newcommand{\iab}{$\mbox{ab}^{-1}$}
% \newcommand{\gvf}{g_V^f}
% \newcommand{\gaf}{g_A^f}

\newcommand{\VCKM}{V_{\rm CKM}}
\newcommand{\bsg}{\ensuremath{\br(B \to X_s \ga)}}
\newcommand{\bsll}{\ensuremath{\br(B \to X_s l^+ l^-)}}
\newcommand{\bmm}{\ensuremath{\br(B_s \to \mu^+\mu^-)}}
\newcommand{\dmbs}{\ensuremath{\De M_{B_s}}}
\newcommand{\gmt}{\ensuremath{(g-2)_\mu}}


\newcommand{\DMh}{\ensuremath{\De \Mh^{\rm MFV}}}
\newcommand{\DMH}{\ensuremath{\De \MH^{\rm MFV}}}
\newcommand{\DMHp}{\ensuremath{\De \MHp^{\rm MFV}}}
\newcommand{\Drho}{\ensuremath{\De\rho^{\rm MFV}}}
\newcommand{\DMW}{\ensuremath{\De\MW^{\rm MFV}}}
\newcommand{\Dsweff}{\ensuremath{\De\sweff^{\rm MFV}}}
\newcommand{\Dbsg}{\ensuremath{\De \br^{\rm MFV}(B \to X_s \gamma)}}
\newcommand{\Dbmm}{\ensuremath{\De \br^{\rm MFV}(B_s \to \mu^+ \mu^-)}}
\newcommand{\Ddmbs}{\ensuremath{\De M_{B_s}^{\rm MFV}}}
\newcommand{\brmeg}{\ensuremath{\br(\mu \to e \ga)}}
\newcommand{\brteg}{\ensuremath{\br(\tau \to e \ga)}}
\newcommand{\brtmg}{\ensuremath{\br(\tau \to \mu \ga)}}


\newcommand{\br}{{\rm BR}}
\newcommand{\CR}{{\rm CR}}
\newcommand{\Dtheo}{\ensuremath{\De^{\rm theo}}}
% \newcommand{\hff}{h \to f\bar{f}}
% \newcommand{\Hff}{H \to f\bar{f}}
% \newcommand{\hbb}{h \to b\bar{b}}
% \newcommand{\Hbb}{H \to b\bar{b}}
% \newcommand{\htautau}{h \to \tau^+\tau^-}
% \newcommand{\hcc}{h \to c\bar{c}}
% \newcommand{\rf}{R_f}
% %\newcommand{\cff}{C_{ff}}
% \newcommand{\cff}{C_f^{(u)}}
% %\newcommand{\cfpfp}{C_{f'f'}}
% \newcommand{\cfpfp}{C_f^{(d)}}
% \newcommand{\Zh}{Z_h}
% \newcommand{\wZh}{\sqrt{\Zh}}
% \newcommand{\ZH}{Z_H}
% \newcommand{\wZH}{\sqrt{\ZH}}
% \newcommand{\ZhH}{Z_{hH}}
% \newcommand{\ZHh}{Z_{Hh}}
% \newcommand{\Zext}{\cZ^{\rm ext}}
% \newcommand{\Zmix}{\cZ^{\rm mix}}
% \newcommand{\rS}{{\rm S\,}}
% \newcommand{\rP}{{\rm P\,}}

\newcommand{\rHiggs}{{\rm Higgs}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmSP}{{\rm SP}}
\newcommand{\rmC}{{\rm C}}

\def\ie{i.e.\ }
\def\eg{e.g.\ }

\def\mpar#1{\marginpar{\tiny #1}}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mda{\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Muua{\marginpar[\boldmath\hfil$\Uparrow\Uparrow$]%
                   {\boldmath$\Uparrow\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mdda{\marginpar[\boldmath\hfil$\Downarrow\Downarrow$]%
                   {\boldmath$\Downarrow\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil$\Rightarrow$]%
                   {\boldmath$\Leftarrow $\hfil}%
                    \typeout{marginpar: $\Leftrightarrow$}\ignorespaces}

%\definecolor{Orange}{named}{Orange}
%\definecolor{Purple}{named}{Purple}
\newcommand{\htr}[1]{{\color{red} #1}}
\newcommand{\htb}[1]{{\color{blue} #1}}
\newcommand{\htg}[1]{{\color{green} #1}}
\newcommand{\htgd}[1]{{\color{green} \st{#1}}}
\newcommand{\hto}[1]{{\color{orange}  #1}}
\newcommand{\htp}[1]{{\color{purple}  #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\oaas}{{\cal O}(\alpha\alpha_s)}
\newcommand{\Gmu}{G_{\mu}}

\newcommand{\hbs}{\ensuremath{h \to \bar b s + b \bar s}}
\newcommand{\brhbs}{\ensuremath{\br(\hbs)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\MSQ[1]{M_{\tilde Q,#1}}
\newcommand\MSU[1]{M_{\tilde U,#1}}
\newcommand\MSD[1]{M_{\tilde D,#1}}
\newcommand\MSL[1]{M_{\tilde L,#1}}
\newcommand\MSR[1]{M_{\tilde R,#1}}
\newcommand\MSX[1]{M_{\tilde X,#1}}
\newcommand\LL{\mathrm{LL}}
\newcommand\LR{\mathrm{LR}}
\newcommand\RL{\mathrm{RL}}
\newcommand\RR{\mathrm{RR}}
\newcommand\uct{\{{u},{c},{t}\}}
\newcommand\dsb{\{{d},{s},{b}\}}
\newcommand\ru{{u}}
\newcommand\rd{{d}}
%\newcommand\deu[2]{\mathtt{#2} &= (\delta_u)_{#1}}
\newcommand\deu[3]{(\delta_{\tinu})_{#1} &:= \del{#2}{#3}}
%\newcommand\ded[2]{\mathtt{#2} &= (\delta_d)_{#1}}
\newcommand\ded[3]{(\delta_{\til})_{#1} &:= \del{#2}{#3}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\stilde{\widetilde}
\def\vspc{\vrule width 0pt height 2.5ex depth 1.5ex}
\def\noent{\vspc~\cdot~}


